Clash of Titans: a MUSE dynamical study of the extreme cluster merger SPT-CL J0307-6225

We present VLT/MUSE spectroscopy, along with archival Gemini/GMOS spectroscopy, Magellan/Megacam imaging, and Chandra X-ray emission for SPT-CL J0305-6225, a z=0.58 major merging galaxy cluster with a large BCG-SZ centroid separation and a highly disturbed X-ray morphology. The galaxy density distribution shows two main overdensities with separations of 0.144 and 0.017 arcmin to their respective BCGs. We characterize the central regions of the two colliding structures, namely 0307-6225N and 0307-6225S, finding velocity derived masses of $M_{200,N}=$ 2.44 $\pm$ 1.41 $\times10^{14}$ M$_\odot$ and $M_{200,S}=$ 3.16 $\pm$ 1.88 $\times10^{14}$ M$_\odot$, with a line-of-sight velocity difference of $|\Delta v| = 342$ km s$^{-1}$. The total dynamically derived mass is consistent with the SZ derived mass of 7.63 h$_{70}^{-1}$ $\pm$ 1.36 $\times10^{14}$ M$_\odot$. We model the merger using the Monte Carlo Merger Analysis Code, estimating a merging angle of 36$^{+14}_{-12}$ degrees with respect to the plane of the sky. Comparing with simulations of a merging system with a mass ratio of 1:3, we find that the best scenario is that of an ongoing merger that began 0.96$^{+0.31}_{-0.18}$ Gyr ago. We also characterize the galaxy population using H$\delta$ and [OII] $\lambda 3727$ \AA \ lines. We find that most of the emission-line galaxies belong to 0307-6225S, close to the X-ray peak position, with a third of them corresponding to red-cluster sequence galaxies, and the rest to blue galaxies with velocities consistent with recent periods of accretion. Moreover, we suggest that 0307-6225S suffered a previous merger, evidenced through the two equally bright BCGs at the center with a velocity difference of $\sim$674 km s$^{-1}$.

==> table_specz_cluster.tex <==
  03:07:16.80 & -62:26:23.12 & MUSE & Cube 1 & 4 & 0.5761 & 25.292 & 23.188 & 22.13 & 2.198 & 1.1\\
  03:07:16.12 & -62:26:25.34 & MUSE & Cube 1 & 6 & 0.5855 & 22.298 & 20.752 & 19.94 & 1.572 & 0.808\\
  03:07:16.02 & -62:26:28.51 & MUSE & Cube 1 & 7 & 0.5716 & 23.813 & 22.289 & 21.487 & 1.412 & 0.816\\
  03:07:14.51 & -62:26:26.89 & MUSE & Cube 1 & 9 & 0.5761 & 24.473 & 22.6 & 21.651 & 1.884 & 0.961\\
  03:07:14.27 & -62:26:30.88 & MUSE & Cube 1 & 13 & 0.578 & 23.503 & 21.574 & 20.718 & 1.915 & 0.868\\
  03:07:15.11 & -62:26:40.05 & MUSE & Cube 1 & 30 & 0.5694 & 21.449 & 21.037 & 20.809 & 0.419 & 0.234\\
  03:07:16.57 & -62:26:41.39 & MUSE & Cube 1 & 35 & 0.5827 & 22.27 & 20.261 & 19.329 & 1.878 & 0.95\\
  03:07:14.87 & -62:26:43.18 & MUSE & Cube 1 & 38 & 0.5729 & 22.122 & 21.722 & 21.598 & 0.393 & 0.104\\
  03:07:13.68 & -62:26:43.71 & MUSE & Cube 1 & 40 & 0.5806 & 24.252 & 22.775 & 21.914 & 1.474 & 0.897\\
  03:07:18.09 & -62:26:45.12 & MUSE & Cube 1 & 42 & 0.5961 & 23.0 & 22.413 & 22.129 & 0.532 & 0.327\\
  03:07:16.23 & -62:26:47.06 & MUSE & Cube 1 & 45 & 0.5813 & 24.609 & 22.317 & 21.333 & 2.235 & 0.979\\
  03:07:16.75 & -62:26:47.43 & MUSE & Cube 1 & 46 & 0.5792 & 22.222 & 20.303 & 19.344 & 1.912 & 0.984\\
  03:07:16.61 & -62:26:49.61 & MUSE & Cube 1 & 47 & 0.574 & 24.553 & 22.549 & 21.6 & 2.008 & 0.95\\
  03:07:19.06 & -62:26:48.68 & MUSE & Cube 1 & 50 & 0.5792 & 25.137 & 22.992 & 22.082 & 2.83 & 0.986\\
  03:07:16.22 & -62:26:50.30 & MUSE & Cube 1 & 51 & 0.5786 & 24.482 & 22.556 & 21.596 & 2.091 & 0.967\\
  03:07:17.62 & -62:26:55.52 & MUSE & Cube 1 & 61 & 0.583 & 25.192 & 23.469 & 22.601 & 2.023 & 0.855\\
  03:07:14.52 & -62:26:55.41 & MUSE & Cube 1 & 63 & 0.592 & 23.568 & 23.349 & 23.142 & 0.133 & 0.179\\
  03:07:20.82 & -62:26:56.46 & MUSE & Cube 1 & 65 & 0.5778 & 24.663 & 22.861 & 21.961 & 1.445 & 0.882\\
  03:07:18.42 & -62:26:59.81 & MUSE & Cube 1 & 69 & 0.5749 & 24.896 & 23.217 & 22.356 & 1.53 & 0.948\\
  03:07:14.37 & -62:27:03.47 & MUSE & Cube 1 & 74 & 0.5879 & 24.141 & 23.651 & 23.327 & 0.493 & 0.225\\
  03:07:15.77 & -62:27:09.28 & MUSE & Cube 1 & 80 & 0.5949 & 22.051 & 21.692 & 21.54 & 0.355 & 0.154\\
  03:07:12.74 & -62:27:10.74 & MUSE & Cube 1 & 82 & 0.5766 & 23.951 & 21.885 & 20.898 & 2.124 & 0.982\\
  03:07:14.87 & -62:27:11.27 & MUSE & Cube 1 & 84 & 0.5855 & 25.151 & 23.06 & 22.152 & 1.918 & 0.96\\
  03:07:15.89 & -62:27:22.14 & MUSE & Cube 1 & 92 & 0.5807 & 24.375 & 22.546 & 21.52 & 1.649 & 1.044\\
  03:07:15.65 & -62:27:22.78 & MUSE & Cube 1 & 93 & 0.5834 & 23.585 & 21.895 & 20.951 & 1.686 & 0.947\\
  03:07:17.20 & -62:25:02.68 & MUSE & Cube 2 & 4 & 0.5787 & 24.702 & 22.803 & 22.021 & 1.968 & 0.811\\
  03:07:17.02 & -62:25:05.38 & MUSE & Cube 2 & 8 & 0.5724 & 24.943 & 23.234 & 22.432 & 1.539 & 0.736\\
  03:07:21.08 & -62:25:13.45 & MUSE & Cube 2 & 17 & 0.585 & 24.04 & 23.281 & 22.917 & 0.74 & 0.186\\
  03:07:16.80 & -62:25:18.55 & MUSE & Cube 2 & 21 & 0.5867 & 24.156 & 23.286 & 23.073 & 0.965 & 0.052\\
  03:07:22.93 & -62:25:18.19 & MUSE & Cube 2 & 23 & 0.5856 & 25.186 & 23.491 & 22.706 & 1.767 & 0.733\\
  03:07:21.73 & -62:25:19.71 & MUSE & Cube 2 & 25 & 0.5829 & 24.928 & 23.157 & 22.273 & 1.763 & 0.933\\
  03:07:21.16 & -62:25:31.01 & MUSE & Cube 2 & 38 & 0.5894 & 22.802 & 21.098 & 20.166 & 1.695 & 0.937\\
  03:07:21.88 & -62:25:36.13 & MUSE & Cube 2 & 48 & 0.5829 & 24.595 & 22.628 & 21.681 & 1.64 & 0.918\\
  03:07:22.26 & -62:25:37.21 & MUSE & Cube 2 & 49 & 0.5749 & 23.628 & 21.943 & 20.991 & 1.698 & 0.956\\
  03:07:17.23 & -62:25:40.65 & MUSE & Cube 2 & 51 & 0.5705 & 24.285 & 22.422 & 21.494 & 1.881 & 0.952\\
  03:07:21.00 & -62:25:36.43 & MUSE & Cube 2 & 55 & 0.5922 & 24.272 & 22.43 & 21.593 & 1.927 & 0.846\\
  03:07:17.81 & -62:25:46.31 & MUSE & Cube 2 & 61 & 0.578 & 23.132 & 21.614 & 20.797 & 1.528 & 0.816\\
  03:07:19.81 & -62:25:45.89 & MUSE & Cube 2 & 63 & 0.591 & 24.26 & 23.52 & 23.285 & 0.959 & -0.01\\
  03:07:16.65 & -62:25:48.66 & MUSE & Cube 2 & 66 & 0.5899 & 25.097 & 23.28 & 22.409 & 2.206 & 0.842\\
  03:07:19.27 & -62:25:48.79 & MUSE & Cube 2 & 67 & 0.5797 & 24.414 & 22.93 & 22.072 & 1.427 & 0.774\\
  03:07:20.70 & -62:25:50.35 & MUSE & Cube 2 & 68 & 0.5786 & 21.944 & 20.67 & 19.892 & 1.313 & 0.837\\
  03:07:16.65 & -62:25:54.11 & MUSE & Cube 2 & 78 & 0.569 & 25.203 & 23.675 & 22.783 & 1.251 & 0.948\\
  03:07:20.69 & -62:25:53.83 & MUSE & Cube 2 & 79 & 0.5797 & 23.168 & 22.083 & 21.708 & 1.079 & 0.406\\
  03:07:17.81 & -62:25:56.62 & MUSE & Cube 2 & 85 & 0.5859 & 23.62 & 21.788 & 20.898 & 1.767 & 0.89\\
  03:07:21.40 & -62:25:58.09 & MUSE & Cube 2 & 87 & 0.5795 & 24.844 & 22.919 & 22.016 & 2.217 & 0.872\\
  03:07:22.17 & -62:26:00.71 & MUSE & Cube 2 & 90 & 0.5736 & 25.099 & 23.136 & 22.234 & 2.199 & 1.002\\
  03:07:22.83 & -62:24:18.61 & MUSE & Cube 3 & 8 & 0.583 & 23.713 & 21.908 & 21.033 & 1.815 & 0.894\\
  03:07:23.40 & -62:24:27.73 & MUSE & Cube 3 & 19 & 0.579 & 23.336 & 21.591 & 20.792 & 1.78 & 0.829\\
  03:07:23.14 & -62:24:29.86 & MUSE & Cube 3 & 23 & 0.5783 & 23.821 & 22.027 & 21.164 & 1.729 & 0.855\\
  03:07:20.55 & -62:24:32.88 & MUSE & Cube 3 & 24 & 0.572 & 24.798 & 23.1 & 22.272 & 1.597 & 0.825\\
  03:07:21.46 & -62:24:42.92 & MUSE & Cube 3 & 34 & 0.5819 & 24.244 & 22.718 & 22.052 & 1.583 & 0.632\\
  03:07:23.09 & -62:24:47.93 & MUSE & Cube 3 & 42 & 0.5753 & 24.943 & 23.012 & 22.102 & 2.12 & 0.92\\
  03:07:20.51 & -62:24:50.94 & MUSE & Cube 3 & 49 & 0.5779 & 23.558 & 22.119 & 21.186 & 1.279 & 0.934\\
  03:07:22.94 & -62:24:59.24 & MUSE & Cube 3 & 58 & 0.5899 & 23.944 & 22.708 & 22.196 & 1.254 & 0.513\\
  03:07:22.83 & -62:25:01.47 & MUSE & Cube 3 & 62 & 0.581 & 24.242 & 23.165 & 22.819 & 0.987 & 0.403\\
  03:07:25.25 & -62:25:03.18 & MUSE & Cube 3 & 64 & 0.5864 & 23.979 & 22.442 & 21.643 & 1.631 & 0.803\\
  03:07:22.16 & -62:25:09.17 & MUSE & Cube 3 & 76 & 0.5725 & 25.233 & 23.313 & 22.376 & 1.834 & 0.945\\
  03:07:21.89 & -62:23:28.04 & MUSE & Cube 4 & 13 & 0.5771 & 22.956 & 21.217 & 20.409 & 1.712 & 0.817\\
  03:07:26.90 & -62:23:28.12 & MUSE & Cube 4 & 14 & 0.586 & 24.507 & 22.764 & 21.955 & 1.719 & 0.821\\
  03:07:30.15 & -62:23:31.80 & MUSE & Cube 4 & 15 & 0.579 & 23.32 & 22.259 & 21.585 & 1.081 & 0.684\\
  03:07:28.25 & -62:23:36.05 & MUSE & Cube 4 & 16 & 0.5867 & 24.186 & 22.344 & 21.405 & 1.873 & 0.945\\
  03:07:26.92 & -62:23:36.95 & MUSE & Cube 4 & 18 & 0.5733 & 24.684 & 22.822 & 21.887 & 1.848 & 0.939\\
  03:07:28.56 & -62:23:37.56 & MUSE & Cube 4 & 19 & 0.5837 & 24.066 & 22.388 & 21.656 & 1.716 & 0.774\\
  03:07:22.44 & -62:23:43.38 & MUSE & Cube 4 & 24 & 0.5803 & 24.648 & 22.691 & 21.821 & 1.54 & 0.8\\
  03:07:26.13 & -62:23:44.20 & MUSE & Cube 4 & 25 & 0.5823 & 24.632 & 22.951 & 22.073 & 1.452 & 0.785\\
  03:07:28.48 & -62:23:44.96 & MUSE & Cube 4 & 26 & 0.5841 & 23.618 & 22.073 & 21.463 & 1.525 & 0.615\\
  03:07:26.77 & -62:23:51.79 & MUSE & Cube 4 & 33 & 0.5759 & 23.908 & 22.16 & 21.28 & 1.667 & 0.888\\
  03:07:25.74 & -62:23:54.13 & MUSE & Cube 4 & 35 & 0.5815 & 23.969 & 22.147 & 21.224 & 1.659 & 0.892\\
  03:07:27.18 & -62:23:54.43 & MUSE & Cube 4 & 37 & 0.5846 & 23.364 & 22.609 & 22.225 & 0.663 & 0.417\\
  03:07:27.50 & -62:23:59.31 & MUSE & Cube 4 & 44 & 0.5779 & 23.718 & 23.318 & 23.221 & 0.445 & -0.117\\
  03:07:24.51 & -62:24:00.96 & MUSE & Cube 4 & 46 & 0.583 & 25.35 & 23.431 & 22.477 & 1.936 & 1.023\\
  03:07:23.86 & -62:24:02.18 & MUSE & Cube 4 & 47 & 0.5802 & 24.326 & 22.439 & 21.528 & 1.89 & 0.934\\
  03:07:24.76 & -62:24:02.30 & MUSE & Cube 4 & 48 & 0.578 & 25.216 & 23.322 & 22.37 & 1.979 & 1.044\\
  03:07:28.06 & -62:24:03.86 & MUSE & Cube 4 & 50 & 0.5819 & 24.889 & 22.947 & 22.14 & 1.978 & 0.73\\
  03:07:28.16 & -62:24:04.95 & MUSE & Cube 4 & 51 & 0.5808 & 25.11 & 22.964 & 22.049 & 2.527 & 0.821\\
  03:07:24.55 & -62:24:06.62 & MUSE & Cube 4 & 54 & 0.5821 & 24.272 & 22.389 & 21.518 & 1.816 & 0.868\\
  03:07:24.18 & -62:24:07.57 & MUSE & Cube 4 & 56 & 0.5753 & 24.073 & 22.237 & 21.278 & 1.844 & 0.938\\
  03:07:23.85 & -62:24:10.12 & MUSE & Cube 4 & 57 & 0.5809 & 21.834 & 19.98 & 19.014 & 1.893 & 0.993\\
  03:07:25.10 & -62:24:11.12 & MUSE & Cube 4 & 60 & 0.5847 & 25.519 & 23.725 & 22.702 & 1.705 & 1.137\\
  03:07:07.53 & -62:24:35.80 & GMOS & Mask 1 & 11 & 0.5837 & 22.64 & 21.539 & 20.904 & 1.102 & 0.65\\
  03:07:29.24 & -62:25:04.10 & GMOS & Mask 1 & 14 & 0.5732 & 23.335 & 22.153 & 21.477 & 1.204 & 0.674\\
  03:07:26.39 & -62:25:37.16 & GMOS & Mask 1 & 15 & 0.5815 & 24.048 & 22.468 & 21.734 & 1.567 & 0.729\\
  03:07:27.26 & -62:25:13.13 & GMOS & Mask 1 & 17 & 0.5807 & 23.876 & 22.555 & 22.108 & 1.283 & 0.444\\
  03:07:21.13 & -62:27:49.79 & GMOS & Mask 1 & 31 & 0.5709 & 22.413 & 21.213 & 20.553 & 1.165 & 0.652\\
  03:07:26.50 & -62:25:18.88 & GMOS & Mask 2 & 10 & 0.5804 & 23.213 & 21.235 & 20.273 & 2.007 & 0.961\\
  03:07:08.71 & -62:24:51.92 & GMOS & Mask 2 & 12 & 0.5752 & 22.124 & 21.322 & 20.898 & 0.792 & 0.42\\
  03:07:36.22 & -62:25:54.68 & GMOS & Mask 2 & 20 & 0.581 & 22.772 & 21.325 & 20.757 & 1.381 & 0.563\\
